3D Reconstruction with Generalizable Neural Fields using Scene Priors

High-fidelity 3D scene reconstruction has been substantially advanced by recent progress in neural fields. However, most existing methods train a separate network from scratch for each individual scene. This is not scalable, inefficient, and unable to yield good results given limited views. While learning-based multi-view stereo methods alleviate this issue to some extent, their multi-view setting makes it less flexible to scale up and to broad applications. Instead, we introduce training generalizable Neural Fields incorporating scene Priors (NFPs). The NFP network maps any single-view RGB-D image into signed distance and radiance values. A complete scene can be reconstructed by merging individual frames in the volumetric space WITHOUT a fusion module, which provides better flexibility. The scene priors can be trained on large-scale datasets, allowing for fast adaptation to the reconstruction of a new scene with fewer views. NFP not only demonstrates SOTA scene reconstruction performance and efficiency, but it also supports single-image novel-view synthesis, which is underexplored in neural fields. More qualitative results are available at: https://oasisyang.github.io/neural-prior

==> figs/optim.tex <==
\begin{figure}[t]
\centering
% \bgroup 
%  \def\arraystretch{0.1} 
%  \setlength\tabcolsep{0.5pt}
%  \begin{tabular}{c}
\includegraphics[width=0.5\textwidth]{figs/optim.png}
% 	\includegraphics[width=0.35\textwidth]{figs/num_frame.png} 
% \end{tabular} \egroup
\vspace{-8mm}
\caption{\small{\textbf{Per-scene optimization.} Upon the scene prior fused from multi-view RGB-D images, we further update it on an individual scene for the better scene reconstruction with prior-guided voxel pruning and point sampling.}}
\label{fig:optim}
\vspace{-4mm}
\end{figure}

==> tables/ablation.tex <==
\begin{figure}
\begin{minipage}{0.5\textwidth}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{2pt}
    \begin{tabular} {c|c|c|c}
    \toprule
    Geo. prior & Acc$\downarrow$ & Comp$\downarrow$ & F-score$\uparrow$ \\ \hlineB{2.5}
    & 0.079 & 0.031 & 0.851  \\ 
     \checkmark & \textbf{0.046} & \textbf{0.030} & \textbf{0.862} \\ \hlineB{2.5}
     Color prior & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS$\downarrow$ \\ \hlineB{2.5}
     & 25.87 & 0.899 & 0.415 \\ 
     \checkmark & \textbf{26.88} & \textbf{0.909} & \textbf{0.246} \\ 
     \bottomrule
    \end{tabular}
    \captionof{table}{\small{{\bf Ablation studies on geometric and texture prior.} We report both mesh reconstruction metrics and novel view synthesis metrics.}}
      \label{tab:calib}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}
  \centering
  \footnotesize
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{lccc}
    \toprule
    \#D  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   \\
    \midrule
    64  & 26.68 & 0.863 & 0.143 \\
    32  & 26.56 & 0.861 & 0.141 \\
    16  & 26.65 & 0.861 & 0.144 \\
    \bottomrule
  \end{tabular}
  \captionof{table}{\small{Novel view synthesis on RealEstate10K with the different number of planes.}}
\label{tab:plane}
\end{minipage}
\hfill
\begin{minipage}{0.3\textwidth}

  \centering
  \footnotesize
  \setlength{\tabcolsep}{2pt}
  \begin{tabular}{cccc}
    \toprule
    ratio  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$   \\
    \midrule
    1.0  & 26.68 & 0.863 & 0.143 \\
    0.8  & 26.61 & 0.860 & 0.145 \\
    0.6 & 26.31 & 0.857 & 0.147 \\
    0.4 & 26.21 & 0.851 & 0.151 \\
    0.2 & 25.52 & 0.834 & 0.161 \\
    % \bottomrule
    \bottomrule
  \end{tabular}
  \vspace{-2mm}
   \captionof{table}{\small{Novel view synthesis on RealEstate10K with different ratios of training data.}}
     \label{tab:data}
\end{minipage}
\vspace{-7mm}
\end{figure}

==> tables/nvs_perscene.tex <==
\begin{table*}[t]\setlength{\tabcolsep}{6pt}
\centering
% \footnotesize
% \small
\begin{tabular} {l|cc|cc|cc|cc}
% \hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{scene 0616} & \multicolumn{2}{c|}{scene 0521}  & \multicolumn{2}{c|}{scene 0000} & \multicolumn{2}{c}{scene 0158} \\ 
% \multicolumn{2}{c|}{scene 0316} & \multicolumn{2}{c|}{scene 0316}  & \multicolumn{2}{c|}{scene 0316}  & \multicolumn{2}{c|}{scene 0316} \\
& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & 
PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\ \hline
% PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & 
% PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\
NSVF & 15.71 & 0.704 & 27.73 & 0.892 & 23.36 & 0.823 & 31.98 & 0.951 \\
SVS & 21.38 & \textbf{0.899} & 27.97 & \textbf{0.924} & 21.39 & \textbf{0.914} & 29.43 & 0.953 \\
NeRF & 15.76 & 0.699 & 24.41 & 0.871 & 18.75 & 0.751 & 29.19 & 0.928  \\
NerfingMVS & 18.07 & 0.748 & 28.07 & 0.901 & 22.10 & 0.880 & 30.55 & 0.948 \\ \hline
Ours & \textbf{24.08} & 0.858 & \textbf{30.35} & 0.921 & \textbf{24.85} & 0.880 & \textbf{32.04} & \textbf{0.955} \\ \hline
\multirow{2}{*}{Methods} & \multicolumn{2}{c|}{scene 0316} & \multicolumn{2}{c|}{scene 0553}  & \multicolumn{2}{c|}{scene 0653} & \multicolumn{2}{c}{scene 0079} \\ 
& PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ & 
PSNR$\uparrow$ & SSIM$\uparrow$ & PSNR$\uparrow$ & SSIM$\uparrow$ \\\hline
NSVF & 22.29 & 0.917 & 31.15 & 0.947 & 28.95 & 0.929 & 26.88 & 0.887 \\
SVS & 20.63 & 0.941 & 30.95 & 0.968 & 27.91 & 0.965 & 25.18 & \textbf{0.923} \\
NeRF & 17.09 & 0.828 & 30.76 & 0.950 & 30.89 & 0.953 & 25.48 & 0.896 \\
NerfingMVS & 20.88 & 0.899 & \textbf{32.56} & \textbf{0.965} & \textbf{31.43} & \textbf{0.964} & 27.27 & 0.916 \\ \hline
Ours & \textbf{27.55} & \textbf{0.950} & 31.46 & 0.960 & 30.35	& 0.952 & \textbf{30.26} & 0.902 \\ 
\end{tabular}
\vspace{-3mm}

\vspace{-3mm}
\label{ab3}
\end{table*}

==> tables/rebuttal_depth.tex <==
\begin{table}[t]\setlength{\tabcolsep}{2pt}
\centering
\scriptsize
% \small
\vspace{-1mm}
\begin{tabular} {l|c|c|c|c}
Method & Abs Rel$\downarrow$ & Sq Rel$\downarrow$ & RMSE$\downarrow$ & $\delta < 1.25 \uparrow $ \\ \hline
NerfingMVS \cite{wei2021nerfingmvs} & 0.0614 & 0.0126 & 0.1345 & 0.9601 \\ 
NerfingMVS$^{*}$ \cite{wei2021nerfingmvs} & 0.0422 & 0.0105 & 0.1157 & 0.9804 \\ 
Go-surf \cite{wang2022go} & 0.0225 & 0.0032 & 0.0773 & 0.9925 \\ \hline
Ours & \textbf{0.0155} & \textbf{0.0021} & \textbf{0.0573} & \textbf{0.9955} 

% \cdashline{1-8}
%  \multicolumn{8}{c}{\bf No Real275 3D Annotations}\\
% \hline
\end{tabular}
\vspace{-3mm}
\caption{\scriptsize{Quantitative comparisons for depth estimation on ScanNet.}}
\vspace{-3mm}
\label{reb:depth}
\end{table}

==> tables/rebuttal_syn.tex <==
\begin{table}[t]\setlength{\tabcolsep}{2pt}
\centering
\scriptsize
% \small
\begin{tabular} {l|c|cc|cc|cc}
% \hline
% \multirow{2}{*}{Methods}  & 
%  \multicolumn{8}{c}{\bf With Real275 3D Annotations}\\
 & & \multicolumn{2}{c|}{breakfast} & \multicolumn{2}{c|}{green room} & \multicolumn{2}{c}{kitchen}\\ \hline
Method & opt. time & NC$\uparrow$ & F-score$\uparrow$ &  NC$\uparrow$ & F-score$\uparrow$ & NC$\uparrow$ & F-score$\uparrow$ \\ 
Neural-RGBD~\cite{azinovic2022neural} & 4hr & 0.934 & 0.920 & \textbf{0.932} & \textbf{0.990} & 0.888 & 0.711 \\
Go-surf~\cite{wang2022go} & 0.6hr & 0.942 & 0.929 & 0.928 & 0.981 & 0.935 & \textbf{0.948} \\ \hline
Ours & $\leq$ 0.3hr & \textbf{0.964} & \textbf{0.986} & 0.929 & 0.983 & \textbf{0.938} & 0.939 \\
% MonoSDF$^*$~\cite{yu2022monosdf} & 10hr & 0.942 & 0.912 & 0.926 \\
% Neural-RGBD~\cite{azinovic2022neural} & 4hr & 0.932 & 0.918 & 0.925 \\ \hline
% Ours & 0.2 hr & {\bf0.947} & {\bf 0.962}	& {\bf 0.954} 
% \cdashline{1-8}
%  \multicolumn{8}{c}{\bf No Real275 3D Annotations}\\
% \hline
\end{tabular}
\vspace{-3mm}
\caption{\scriptsize{Quantitative comparisons for mesh reconstruction on Synthetic dataset.}}
\vspace{-6mm}
\label{reb:syn}
\end{table}

==> tables/sota_depth.tex <==
\begin{table}[t]\setlength{\tabcolsep}{2pt}
\centering
\footnotesize
% \small
\begin{tabular} {l|c|c|c|c}
% Method & Abs Rel$\downarrow$ & Sq Rel$\downarrow$ & RMSE$\downarrow$ & RMSE log$\downarrow$ & $\delta < 1.25 \uparrow $  & $\delta < 1.25^2 \uparrow$ & $\delta < 1.25^3 \uparrow$ \\ \hline
% 	COLMAP \cite{schonberger2016structure,schonberger2016pixelwise}& 0.4619 &0.6308 &1.0125 &1.7345 &0.4811 &0.5139 &0.5333 
%     \\
%     ACMP \cite{xu2020planar}&  0.1945 &0.1710 &0.4551 &0.3056 &0.7309 &0.8810 &0.9419 
%     \\			\hline
%     DELTAS \cite{sinha2020deltas}&0.1001 &0.0319 &0.2070 &0.1284 &0.8618 &0.9920 &0.9991 
%     \\
%     Atlas \cite{murez2020atlas}&0.0776 &0.0631 &0.2441 &0.2693 &0.9289 &0.9536 &0.9594
%     \\
%     DeepV2D \cite{teed2018deepv2d} & 0.0818 &0.0226 &0.1714 &0.1095 &0.9414 &0.9908 &0.9979 
%     \\			\hline
%     NeRF \cite{mildenhall2020nerf}&0.3929 &1.4849 &1.0901 &0.5210 &0.4886 &0.7318 &0.8285 
%     \\
%     Mannequin \cite{li2019learning}&0.1554 &0.0636 &0.2969 &0.1806 &0.7859 &0.9735 &0.9953 
%     \\
%     CVD \cite{luo2020consistent}&0.0995 &0.0304 &0.1945 &0.1269 &0.9008 &0.9879 & 0.9971 \\
%     % NerfingMVS w/o filter & 0.0635 &0.0145 &0.1455 &0.0936 &0.9541 &0.9910 &0.9989 \\ 
%     NerfingMVS \cite{wei2021nerfingmvs} & 0.0614 & 0.0126 & 0.1345 & 0.0861 & 0.9601 & 0.9955 & 0.9996 \\ \hline
%     Ours & \textbf{0.0155} & \textbf{0.0021} & \textbf{0.0573} & \textbf{0.0343} & \textbf{0.9955} & \textbf{0.9993} & \textbf{0.9999} 


Method & Abs Rel$\downarrow$ & Sq Rel$\downarrow$ & RMSE$\downarrow$ & $\delta < 1.25 \uparrow $ \\ \hline
	% COLMAP \cite{schonberger2016structure,schonberger2016pixelwise}& 0.4619 &0.6308 &1.0125  &0.4811 
 %    \\
 %    ACMP \cite{xu2020planar}&  0.1945 &0.1710 &0.4551  &0.7309 
 %    \\			\hline
    % DELTAS \cite{sinha2020deltas}&0.1001 &0.0319 &0.2070  &0.8618 
    % \\
    % Atlas \cite{murez2020atlas}&0.0776 &0.0631 &0.2441  &0.9289 
    % \\
    % DeepV2D \cite{teed2018deepv2d} & 0.0818 &0.0226 &0.1714 &0.9414 
    % \\			\hline
    NeRF \cite{mildenhall2020nerf}&0.3929 &1.4849 &1.0901 &0.4886 
    \\
    % Mannequin \cite{li2019learning}&0.1554 &0.0636 &0.2969  &0.7859 
    % \\
    CVD \cite{luo2020consistent}&0.0995 &0.0304 &0.1945 &0.9008  
    \\
    % NerfingMVS w/o filter & 0.0635 &0.0145 &0.1455 &0.0936 &0.9541 &0.9910 &0.9989 \\ 
    NerfingMVS \cite{wei2021nerfingmvs} & 0.0614 & 0.0126 & 0.1345 & 0.9601 \\ 
    NerfingMVS$^{*}$ \cite{wei2021nerfingmvs} & 0.0422 & 0.0105 & 0.1157 & 0.9804 \\ 
    Go-surf \cite{wang2022go} & 0.0225 & 0.0032 & 0.0773 & 0.9925 \\ \hline
    Ours & \textbf{0.0155} & \textbf{0.0021} & \textbf{0.0573} & \textbf{0.9955} 

% \cdashline{1-8}
%  \multicolumn{8}{c}{\bf No Real275 3D Annotations}\\
% \hline
\end{tabular}
\vspace{-3mm}
\caption{\small{{\bf Quantitative comparisons for multi-view depth estimation on ScanNet.} We evaluate the depth error on the unseen views during inference. Our method, without the post-filtering step, outperforms all compared methods.}}
\vspace{-6mm}
\label{sota:depth}
\end{table}

==> tables/sota_fusion.tex <==
\begin{table}\setlength{\tabcolsep}{4pt}
\centering
% \footnotesize
% \small
\begin{tabular} {l|c|c|c}
% \hline
% \multirow{2}{*}{Methods}  & 
%  \multicolumn{8}{c}{\bf With Real275 3D Annotations}\\
Method & Prec$\uparrow$ & Recall$\uparrow$ & F-score$\downarrow$ \\ \hline
TSDF Fusion & 0.738 & 0.859 &  0.788 \\
iMAP & 0.690 0.821 & 0.750 \\
DI Fusion & 0.663 & 0.797 & 73.0 \\
BNVF & 0.749 & 0.881 & 0.806 \\
Ours & \textbf{26.88} & \underline{0.909} & \underline{0.246}\\
% Go-surf$_{30 min}$ & 0.0515	0.0176	0.9464	0.9556	0.9504
% Ours$_{10 min}$ & 0.0488	0.0166	0.9474	0.9618	0.9542
% Ours & 0.048 & 0.017 & 0.947 & 0.962 & 0.9542 \\\hline


% \cdashline{1-8}
%  \multicolumn{8}{c}{\bf No Real275 3D Annotations}\\
% \hline
\end{tabular}
\vspace{-3mm}
\caption{{\bf }}
\vspace{-4mm}
\label{sota:nvs}
\end{table}
